Style Variable and Irrelevant Learning for Generalizable Person Re-identification

Recently, due to the poor performance of supervised person re-identification (ReID) to an unseen domain, Domain Generalization (DG) person ReID has attracted a lot of attention which aims to learn a domain-insensitive model and can resist the influence of domain bias. In this paper, we first verify through an experiment that style factors are a vital part of domain bias. Base on this conclusion, we propose a Style Variable and Irrelevant Learning (SVIL) method to eliminate the effect of style factors on the model. Specifically, we design a Style Jitter Module (SJM) in SVIL. The SJM module can enrich the style diversity of the specific source domain and reduce the style differences of various source domains. This leads to the model focusing on identity-relevant information and being insensitive to the style changes. Besides, we organically combine the SJM module with a meta-learning algorithm, maximizing the benefits and further improving the generalization ability of the model. Note that our SJM module is plug-and-play and inference cost-free. Extensive experiments confirm the effectiveness of our SVIL and our method outperforms the state-of-the-art methods on DG-ReID benchmarks by a large margin.

==> tab/dataset.tex <==
\begin{table}[h]
\tabcolsep=2pt
\centering
\caption{Details about the ReID benchmarks.
	}
\small
  \begin{tabular}{c|c|c|c|c}
  \hline
  Datasets & Images & Identities & Cameras & Scene \\
  \hline
  Market1501 \cite{zheng2015scalable} & 32668 & 1501 & 6 & outdoor \\ 
  DukeMTMC-reID \cite{zheng2017unlabeled} & 32948 & 1404 & 8 & outdoor\\
  CUHK03 \cite{li2014deepreid} & 28192 & 1467 & 2 & indoor\\
  MSMT17 \cite{wei2018person} & 126142 & 4101 & 15 & in \& out\\
  \hline
  \end{tabular}
  \label{tab:dataset}
\end{table}

==> tab/scale.tex <==
\begin{table}[ht]
% \tabcolsep=3pt
\small
\centering
\caption{Comparison with different scales in the SRJ module.
	}
  \begin{tabular}{c|cc|cc}
  \hline
	\multirow{2}{*}{Method} & \multicolumn{2}{c|}{C+D+MS$\rightarrow$M} & \multicolumn{2}{c}{C+M+MS$\rightarrow$D} \\ 
	\cline{2-5}
	& mAP & Rank-1 & mAP & Rank-1 \\ \hline
  % DEMO $^*$ & \multirow{10}{*}{C2+C3+D+M+CS} & TIP 2019 & - & - & - & - & - & - & - & -  \\
  Strong Baseline & 62.30 & 83.43 & 60.72 & 76.26 \\
  \hline
  SRJ (scale=1) & 64.02 & 85.48 & 61.68 & 77.33 \\
  SRJ (scale=2) & 64.56 & 85.66 & 61.47 & 77.06 \\
  SRJ (scale=4) & 64.95 & 86.05 & 61.74 & 77.33 \\
  SRJ (scale=8) & 64.29 & 85.50 & 61.27 & 76.84 \\
  \hline
  \end{tabular}
  \label{tab:scale}
\end{table}

==> tab/sota.tex <==
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccc@{}}
% \toprule
% Method & Frobnability & Frobnability & Frobnability \\
% \midrule
% Theirs & Frumpy \\
% Yours & Frobbly \\
% Ours & Makes one's heart Frob\\
% \bottomrule
% \end{tabular}
% } % \resizebox
% \caption{
% % 
% \textbf{State of the art} -- Glory to the bold numbers.
% % 
% } % \caption
% \label{tab:sota}
% \end{table}
